Distributed quantum incompatibility

Incompatible, i.e. non-jointly measurable quantum measurements are a necessary resource for many information processing tasks. It is known that increasing the number of distinct measurements usually enhances the incompatibility of a measurement scheme. However, it is generally unclear how large this enhancement is and on what it depends. Here, we show that the incompatibility which is gained via additional measurements is upper and lower bounded by certain functions of the incompatibility of subsets of the available measurements. We prove the tightness of some of our bounds by providing explicit examples based on mutually unbiased bases. Finally, we discuss the consequences of our results for the nonlocality that can be gained by enlarging the number of measurements in a Bell experiment.

==> mymath.tex <==
%for process_tom.tex

% ----- new thm environments ------
% \newtheorem{theorem}{Theorem}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{observation}[theorem]{Observation}
% \newtheorem{problem}[theorem]{Problem}

%%%================================================
%%%==============  new commands  =======================
%%%================================================
%------- smaller space in,e.g., $\exp\left(x\right)$
% \let\originalleft\left
% \let\originalright\right
% \renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
% \renewcommand{\right}{\aftergroup\egroup\originalright}
\newcommand{\myleft}{\mathopen{}\mathclose\bgroup\left}
\newcommand{\myright}{\aftergroup\egroup\right}
%%% ------ rm ---------
\newcommand{\e}{\ensuremath\mathrm{e}}
\renewcommand{\i}{\ensuremath\mathrm{i}}
\newcommand{\id}{\ensuremath\mathrm{id}}
\newcommand{\rmd}{\ensuremath\mathrm{d}}
\DeclareMathOperator{\Tr}{Tr}
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\DeclareMathOperator{\ran}{ran}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\vecmap}{vec}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\spec}{spec}
\DeclareMathOperator{\dist}{dist}
\newcommand{\fro}{\mathrm{F}}
\newcommand{\conv}{\operatorname{conv}}
\DeclareMathOperator{\cone}{\operatorname{cone}}
\DeclareMathOperator{\lin}{\operatorname{lin}}

\DeclareMathOperator{\Pos}{Pos}
\DeclareMathOperator{\CPT}{CPT}
\DeclareMathOperator{\Herm}{Herm}
\DeclareMathOperator{\HT}{HT}%hermiticity and trace preserving
\DeclareMathOperator{\TP}{TP}
%\DeclareMathOperator{\HP}{HP}
\newcommand{\Sym}{\mathrm{Sym}}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Choi}{Choi}

\DeclareMathOperator{\U}{U}%unitary group U(n)
\renewcommand{\O}{\operatorname{O}}%orthogonal group U(n)
\DeclareMathOperator{\SU}{SU}%special unitary group SU(n)

%%% -------- Landau symbols ---------
\DeclareMathOperator{\LandauO}{\mathrm{O}}
\DeclareMathOperator{\tLandauO}{\tilde{\mathrm{O}}}
\DeclareMathOperator{\LandauOmega}{\Omega}


%%% ------- complexity -----------
\usepackage{complexity}%customized
% \newcommand{\NP}{\ComplexityFont{NP}}
\renewcommand{\P}{\ComplexityFont{P}}
\newcommand{\sharpP}{\#\ComplexityFont{P}}


%%% ------ mathbb --------
\newcommand{\CC}{\mathbb{C}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\KK}{\mathbb{K}}% for \RR or \CC
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\1}{\mathbb{1}}
% \newcommand{\EE}{\mathbb{E}}
% \newcommand{\PP}{\mathbb{P}}


%%% ------ mathcal ---------
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\X}{\mc{X}}
\newcommand{\Y}{\mc{Y}}
\newcommand{\V}{\mc{V}}
% \newcommand{\W}{\mc{W}}
\newcommand{\F}{\mc{F}}
% \newcommand{\K}{\mc{K}}
\newcommand{\mcM}{\mc{M}}
\newcommand{\mcL}{\mc{L}}
\newcommand{\mcR}{\mc{R}}
\renewcommand{\H}{\mc{H}}


%%% ------ other ----------
\newcommand{\kw}[1]{\frac{1}{#1}}
\newcommand{\tkw}[1]{\tfrac{1}{#1}}
\newcommand{\argdot}{{\,\cdot\,}}
\renewcommand{\vec}[1]{\boldsymbol{#1}}
\providecommand{\DC}{\operatorname{\mathscr{D}}} %descent cone
\newcommand{\ad}{^\dagger}%symbol for conjugate transpose
\renewcommand{\L}{\operatorname{\mathrm{L}}}%linear operators
\newcommand{\LL}{\operatorname{\mathbb{L}}}%linear maps on operators
% \newcommand{\M}{\operatorname{\mathbb{L}}}
\newcommand{\DM}{\operatorname{\mc{D}}} %density operators
\newcommand{\qqquad}{\qquad\qquad}
\newcommand{\dunion}{\,\dot{\cup}\,}


%%% ------ norms, inner product ----------
\newcommand{\norm}[1]{\left\Vert #1 \right\Vert} %norm with variable height
\newcommand{\normn}[1]{\lVert #1 \rVert} %norm with normalsize height
\newcommand{\normb}[1]{\bigl\Vert #1 \bigr\Vert} %norm with big height
\newcommand{\normB}[1]{\Bigl\Vert #1 \Bigr\Vert} %norm with Big height
\newcommand{\snorm}[1]{\norm{#1}_\infty} %spectral norm  =  (2->2)-norm
\newcommand{\snormn}[1]{\normn{#1}_\infty}
\newcommand{\snormb}[1]{\normb{#1}_\infty}
\newcommand{\snormB}[1]{\normB{#1}_\infty}
\newcommand{\tnorm}[1]{\norm{#1}_{1}} %trace norm
\newcommand{\tnormn}[1]{\normn{#1}_{1}}
\newcommand{\tnormb}[1]{\normb{#1}_{1}}
\newcommand{\TrNorm}[1]{\norm{#1}_{1}} %trace norm
\newcommand{\TrNormn}[1]{\normn{#1}_{1}}
\newcommand{\TrNormb}[1]{\normb{#1}_{1}}
\newcommand{\pNorm}[1]{\norm{#1}_p} %diamond norm
\newcommand{\pNormn}[1]{\normn{#1}_p}
\newcommand{\pNormb}[1]{\normb{#1}_p}
\newcommand{\fnorm}[1]{\norm{#1}_\fro} %Frobenius norm
\newcommand{\fnormn}[1]{\normn{#1}_\fro}
\newcommand{\fnormb}[1]{\normb{#1}_\fro}
%\newcommand{\nnorm}[1]{\norm{#1}_1} %nuclear norm
%\newcommand{\nnormn}[1]{\normn{#1}_1}
%\newcommand{\nnormb}[1]{\normb{#1}_1}
\newcommand{\dnorm}[1]{\norm{#1}_\diamond} %diamond norm
\newcommand{\dnormn}[1]{\normn{#1}_\diamond}
\newcommand{\dnormb}[1]{\normb{#1}_\diamond}
\newcommand{\jnorm}[1]{\norm{#1}_\mysquare} % \jnorm{J(M)}=dim(V)*\dnorm{M}
\newcommand{\jnormn}[1]{\normn{#1}_\mysquare}
\newcommand{\jnormb}[1]{\normb{#1}_\mysquare}
\newcommand{\threenorm}[1]{\lvert\lvert\lvert#1\rvert\rvert\rvert} % ||| . |||
\newcommand{\lTwoNorm}[1]{\norm{#1}_{\ell_2}} %\ell_2 norm
\newcommand{\lTwonormn}[1]{\normn{#1}_{\ell_2}}
\newcommand{\lTwonormb}[1]{\normb{#1}_{\ell_2}}
\newcommand{\lqNorm}[1]{\norm{#1}_{\ell_q}} %\ell_q norm
\newcommand{\lqnormn}[1]{\normn{#1}_{\ell_q}}
\newcommand{\lqnormb}[1]{\normb{#1}_{\ell_q}}
\newcommand{\TwoNorm}[1]{\norm{#1}_{2}} % 2 norm
\newcommand{\TwoNormn}[1]{\normn{#1}_{2}}
\newcommand{\TwoNormb}[1]{\normb{#1}_{2}}

%%% ---- Kets -----
\newcommand{\ket}[1]{\left.\left|{#1}\right.\right\rangle}
\newcommand{\ketn}[1]{| #1 \rangle}
\newcommand{\ketb}[1]{\bigl| #1 \bigr\rangle}
\newcommand{\bra}[1]{\left.\left\langle{#1}\right.\right|}
\newcommand{\bran}[1]{\langle #1 |}
\newcommand{\brab}[1]{\bigl\langle #1 \bigr|}
\newcommand{\braket}[2]{\left\langle #1 \middle| #2 \right\rangle}
\newcommand{\braketn}[2]{\langle #1 \middle| #2 \rangle}
\newcommand{\ketbra}[2]{\ket{#1} \!\! \bra{#2}}
\newcommand{\ketibra}[3]{\ket{#1}_{#2} \!\! \bra{#3}}
\newcommand{\ketbran}[2]{\ketn{#1} \! \bran{#2}}
\newcommand{\ketbrab}[2]{\ketb{#1} \! \brab{#2}}
\newcommand{\sandwich}[3]
  {\left\langle  #1 \right| #2 \left| #3 \right\rangle}
\newcommand{\sandwichb}[3]
  {\bigl\langle  #1 \bigr| #2 \bigl| #3 \bigr\rangle}

%%% ------ specific to this project ----------
\renewcommand{\Pr}{\operatorname{\PP}} 
\newcommand{\Ev}{\operatorname{\EE}} %expectation value
% \newcommand{\A}{\mc{A}} %measurement map
\newcommand{\ev}{e} %error vector
\providecommand{\DC}{\operatorname{\mathscr{D}}} %descent cone
\newcommand{\st}{\mathrm{subject\ to}}
\newcommand{\Haar}{\mathrm{Haar}}
% \newcommand{\minimize}{\mathrm{minimize }}
\DeclareMathOperator*{\minimize}{minimize}
\newcommand{\maximize}{\mathrm{maximize }}
\newcommand{\Span}[1]{\langle #1 \rangle}
\newcommand{\mysquare}{{\protect\scalebox{0.5}{$\square$}}}
%\newcommand{\fd}{f_{\mysquare}}
%\newcommand{\J}{$\mysquare$}
\renewcommand{\r}{_{|r}}
\renewcommand{\c}{_{\neg r}}
\newcommand{\rec}{\mathrm{rec}}
\newcommand{\Toff}{\mathrm{Toff}}
\newcommand{\dep}{\mathrm{dep}}
\newcommand{\eps}{\mathrm{eps}}

\newcommand{\Favg}{F_\mathrm{avg}}
%% ----- algorithmic customisation ------------

% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}


